GO4Align: Group Optimization for Multi-Task Alignment

This paper proposes \textit{GO4Align}, a multi-task optimization approach that tackles task imbalance by explicitly aligning the optimization across tasks. To achieve this, we design an adaptive group risk minimization strategy, comprising two techniques in implementation: (i) dynamical group assignment, which clusters similar tasks based on task interactions; (ii) risk-guided group indicators, which exploit consistent task correlations with risk information from previous iterations. Comprehensive experimental results on diverse benchmarks demonstrate our method's performance superiority with even lower computational costs.

==> table/cityscapes.tex <==
\begin{wraptable}{r}{0.5\textwidth}
    \centering
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{lrrrrrrrr}
    \toprule
   \multirow{4}{*}{\textbf{Method}} & \multicolumn{6}{c}{\textbf{CityScapes}} & \multicolumn{2}{c}{\textbf{CelebA}} \\
      \cmidrule(lr){2-7}\cmidrule(lr){8-9}
      &  \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multirow{2}{*}{\mr{} $\downarrow$} & \multirow{2}{*}{ \dm{} $\downarrow$}  & \multirow{2}{*}{\mr{} $\downarrow$} & \multirow{2}{*}{ \dm{} $\downarrow$}\\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}
     &  mIoU $\uparrow$ & Pix Acc $\uparrow$ & Abs Err $\downarrow$ & Rel Err $\downarrow$ &  &  & &\\
    \midrule 
    \stl{}      & 74.01 & 93.16 & 0.0125 & 27.77 & & \\
    \midrule
    \mgda{}     & 68.84 & 91.54 & 0.0309 & 33.50 & 10.75 & 44.14  & 10.90 & 14.85\\
    \pcgrad{}   & 75.13 & 93.48 & 0.0154 & 42.07 & 6.75 & 18.29  & 6.43 & 3.17 \\
    \graddrop{} & 75.27 & 93.53 & 0.0157 & 47.54 & 6.00 & 23.73  & 7.60 & 3.29\\
    \cagrad{}   & 75.16 & 93.48 & 0.0141 & 37.60 & 5.50 & 11.64  & 5.95 & 2.48 \\
    \imtlg{}    & 75.33 & 93.49 & 0.0135 & 38.41 & 4.25 & 11.10  & 4.25 & \best{0.84}\\
    \nashmtl{}  & \best{75.41} & \best{93.66} & \best{0.0129} & 35.02 & \best{2.50} & 6.82  & 4.53 & 2.84 \\
    \midrule
    \ls{}       & 70.95 & 91.73 & 0.0161 & 33.83 & 9.25 & 14.11 & 6.00 & 4.15  \\
    \si{}       & 70.95 & 91.73 & 0.0161 & 33.83 & 9.25 & 14.11 & 7.65 & 7.20  \\
    \rlw{}      & 74.57 & 93.41 & 0.0158 & 47.79 & 8.75 & 24.38 & 4.93 & 1.46  \\
    \dwa{}      & 75.24 & 93.52 & 0.0160 & 44.37 & 6.75 & 21.45 & 6.65 & 3.20  \\
    \uw{}       & 72.02 & 92.85 & 0.0140 & 30.13 & 6.25 & \best{5.50} & 5.78 & 3.23 \\
    \famo{}     & 74.54 & 93.29 & 0.0145 & 32.59 & 6.00  & 8.13 & 4.33 & 1.21  \\
    \ours{} &72.63 &93.03 &0.0164 &\best{27.58} &7.75 &8.11 &\best{3.30} &0.88\\
    \bottomrule 
    \end{tabular}
    }
    \vspace{2pt}
    \caption{Results on CityScapes (2 tasks) and CelebA (40 tasks) datasets. Each experiment is repeated over 3 random seeds and the mean is reported. The best average result is marked in bold. \mr{} and \dm{} are the main metrics for MTL performance.}
    \label{tab: cityscapes-and-celeba}
    \vspace{-20pt}
\end{wraptable}




==> table/codes.tex <==
\usemintedstyle{manni}

\begin{minted}[
frame=lines,
framesep=2mm,
baselinestretch=1.2,
bgcolor=LightGray,
fontsize=\footnotesize,
linenos
]{python}

import torch
import torch.nn.functional as F
from kmeans_pytorch import kmeans

class GO4Align(WeightMethod):
    def __init__(
            self,
            n_tasks: int,
            device: torch.device,
            num_groups: int,
            task_weights: Union[List[float], torch.Tensor] = None,
            beta: float = 0.0001,
    ):
        super().__init__(n_tasks, device=device)
        self.n_tasks = n_tasks
        self.device = device
        if task_weights is None:
            task_weights = torch.ones((n_tasks,))
        if not isinstance(task_weights, torch.Tensor):
            task_weights = torch.tensor(task_weights)
        assert len(task_weights) == n_tasks
        self.task_weights = task_weights.to(device)

        self.adv_probs = torch.ones(n_tasks).to(device) / n_tasks
        self.beta = beta
        self.num_groups = num_groups

    def get_weighted_loss(self, losses, **kwargs):
        adjusted_loss = losses.detach()
        scale = adjusted_loss.sum() / adjusted_loss
        self.adv_probs = self.adv_probs * torch.exp(- self.beta * adjusted_loss)
        self.adv_probs = self.adv_probs / (self.adv_probs.sum())
        weight = scale * self.adv_probs

        weight = weight.unsqueeze(1)

        cluster_ids_x, cluster_centers = kmeans(X=weight, num_clusters=
        self.num_groups, distance='euclidean', device=self.device)
        mask = torch.zeros(self.n_tasks, self.num_groups).to(self.device)
        cluster_ids = cluster_ids_x.unsqueeze(1).to(self.device)
        cluster_centers = cluster_centers.to(self.device)
        mask.scatter_(1, cluster_ids, 1)
        kmeans_weight = torch.mm(mask,cluster_centers).squeeze(1)

        loss = torch.sum(losses * kmeans_weight)
        return loss, dict(weights=torch.cat([kmeans_weight]))
\end{minted}
